Partially Stochastic Infinitely Deep Bayesian Neural Networks

In this paper, we present Partially Stochastic Infinitely Deep Bayesian Neural Networks, a novel family of architectures that integrates partial stochasticity into the framework of infinitely deep neural networks. Our new class of architectures is designed to improve the computational efficiency of existing architectures at training and inference time. To do this, we leverage the advantages of partial stochasticity in the infinite-depth limit which include the benefits of full stochasticity e.g. robustness, uncertainty quantification, and memory efficiency, whilst improving their limitations around computational complexity. We present a variety of architectural configurations, offering flexibility in network design including different methods for weight partition. We also provide mathematical guarantees on the expressivity of our models by establishing that our network family qualifies as Universal Conditional Distribution Approximators. Lastly, empirical evaluations across multiple tasks show that our proposed architectures achieve better downstream task performance and uncertainty quantification than their counterparts while being significantly more efficient. The code can be found at \url{https://github.com/Sergio20f/part_stoch_inf_deep}

==> proof_lemma1.tex <==

\subsection{Proof of Lemma \ref{lemma:KL-diffusion}}
    We calculate the KL-divergence as in \cite{xu2022infinitely}. We let $w_{0}$ be a fixed initial state and $w_{1}, \ldots, w_{N}$ be states at times $t_1 = \Delta t,t_2 =  2 \Delta t, \ldots,t_N = N \Delta t=T$ generated by the Euler discretisation:
    $$
\begin{aligned}
w_{i+1} & =w_{i}+f_{q}\left(t_i,w_{i}\right) \Delta t+\sigma_q\left(t_i,w_{i}\right)\left(B_{t+\Delta t}-B_{t}\right) \\
& =w_{i}+f_{q}\left(t_i,w_{i}\right) \Delta t+\sigma_q\left(t_i,w_{i}\right) \Delta t^{1 / 2} \epsilon_{i+1}
\end{aligned}
$$
where $\epsilon_{i+1} \sim \mathcal{N}(0,1)$. Therefore,
$$
w_{i+1} \mid w_{i} \sim \mathcal{N}\left(w_{i}+f_{q}\left(t_i,w_{i}\right) \Delta t, \sigma_q\left(t_i,w_{i}\right)^{2} \Delta t\right)
$$
and we can write:
$$
\begin{aligned}
\log q\left(w_{i+1} \mid w_{i}\right)=&-\frac{1}{2} \log \left(2 \pi \sigma_q\left(t_i,w_{i}\right)^{2} \Delta t\right)-\frac{1}{2} \frac{\left(w_{i+1}-\left(w_{i}+f_{q}\left(t_i,w_{i}\right) \Delta t\right)\right)^{2}}{\sigma_q\left(t_i,w_{i}\right)^{2} \Delta t}
\end{aligned}
$$
Similarly, for the prior process, we can write:
$$
\begin{aligned}
\log p\left(w_{i+1} \mid w_{i}\right)=&-\frac{1}{2} \log \left(2 \pi \sigma_p\left(t_i,w_{i}\right)^{2} \Delta t\right)-\frac{1}{2} \frac{\left(w_{i+1}-\left(w_{i}+f_{p}\left(t_i,w_{i}\right) \Delta t\right)\right)^{2}}{\sigma_p\left(t_i,w_{i}\right)^{2} \Delta t}
\end{aligned}
$$
By substituting the expression of $w_{i+1}$ into the above equations we get:
$$
\begin{aligned}
\log q\left(w_{i+1} \mid w_{i}\right)= & -\frac{1}{2} \log \left(2 \pi \sigma_q\left(t_i,w_{i}\right)^{2} \Delta t\right)-\frac{1}{2} \epsilon_{i+1}^{2} \\
\log p\left(w_{i+1} \mid w_{i}\right)= & -\frac{1}{2} \log \left(2 \pi \sigma_p\left(t_i,w_{i}\right)^{2} \Delta t\right)  -\frac{1}{2}\Bigg(\frac{\left(f_{q}\left(t_i,w_{i}\right)-f_{p}\left(t_i,w_{i}\right)\right)^{2}}{\sigma_p\left(t_i,w_{i}\right)^{2}} \Delta t\\
&+\frac{2\left(f_{q}\left(t_i,w_{i}\right)-f_{p}\left(t_i,w_{i}\right)\right)\sigma_q\left(t_i,w_{i}\right) \epsilon_{i+1}}{\sigma_p\left(t_i,w_{i}\right)^2} \Delta t^{1 / 2}+\frac{\sigma_q(t_i,w_i)^2}{\sigma_p(t_i,w_i)^2}\epsilon_{i+1}^{2}\Bigg) 
\end{aligned}
$$
Then, the KL-divergence for the discretised process is:
$$
\begin{aligned}
&\sum_{i=0}^{N} \mathbb{E}_{w_{i}}\left[D_{\mathrm{KL}}\left(q\left(w_{i+1} \mid w_{i}\right) \| p\left(w_{i+1} \mid w_{i}\right)\right)\right] \\
= &\sum_{i=0}^{N} \mathbb{E}_{w_{i}}\left[\mathbb{E}_{w_{i+1} \sim q\left(w_{i+1} \mid w_{i}\right)}\left[\log \frac{q\left(w_{i+1} \mid w_{i}\right)}{p\left(w_{i+1} \mid w_{i}\right)}\right]\right] \\
= &\sum_{i=0}^{N} \mathbb{E}_{w_{i}}\Bigg[\mathbb{E}_{\epsilon_{i+1}}\Bigg[A(w_i) \Delta t+B(w_i)\Delta t^{1 / 2} \epsilon_{i+1}\\
&+\frac{1}{2}\left(\frac{\sigma_q(t_i,w_i)^2}{\sigma_p(w_i)^2}-1\right)\epsilon_{i+1}^2-\frac{1}{2}\log\left(\frac{\sigma_q(t_i,w_i)^2}{\sigma_p(t_i,w_i)^2}\right)\Bigg]\Bigg] \\
=&\sum_{i=0}^{N} \mathbb{E}_{w_{i}}\Bigg[A(w_i) \Delta t+\frac{1}{2}\left(\frac{\sigma_q(t_i,w_i)^2}{\sigma_p(t_i,w_i)^2}-1\right)-\frac{1}{2}\log\left(\frac{\sigma_q(t_i,w_i)^2}{\sigma_p(t_i,w_i)^2}\right)\Bigg] \\
\end{aligned}
$$
Now, taking the derivative of the function $f(x)=x^2-1-2\log(x)$ we can see that it has a single minimum point at $x=1$ where $f(1)=0$. Therefore, if \(\sigma_p(t,w_t) \neq \sigma_q(t,w_t)\) with non-zero probability, then
$$
\mathbb E _{w_t}\left[\frac{1}{2}\left(\frac{\sigma_q(t,w_t)^2}{\sigma_p(t,w_t)^2}-1\right)-\frac{1}{2}\log\left(\frac{\sigma_q(t,w_t)^2}{\sigma_p(t,w_t)^2}\right)\right] > 0
$$ 
The left-hand side is actually a continuous function of \(t\) only, call it \(e(t)\).
Since \(e(t)\) is continuous, if we take $N\rightarrow\infty$, the terms \(e(t_i)\) in the neighborhood of \(t\) accumulate and make the sum blow to infinity, i.e $D_{\mathrm{KL}}\left(\mu_{q} \| \mu_{p}\right)=\infty$. \qed 

